UGC: Unified GAN Compression for Efficient Image-to-Image Translation

Recent years have witnessed the prevailing progress of Generative Adversarial Networks (GANs) in image-to-image translation. However, the success of these GAN models hinges on ponderous computational costs and labor-expensive training data. Current efficient GAN learning techniques often fall into two orthogonal aspects: i) model slimming via reduced calculation costs; ii)data/label-efficient learning with fewer training data/labels. To combine the best of both worlds, we propose a new learning paradigm, Unified GAN Compression (UGC), with a unified optimization objective to seamlessly prompt the synergy of model-efficient and label-efficient learning. UGC sets up semi-supervised-driven network architecture search and adaptive online semi-supervised distillation stages sequentially, which formulates a heterogeneous mutual learning scheme to obtain an architecture-flexible, label-efficient, and performance-excellent model.

==> tables/cmp_with_sota_2.tex <==
\begin{table*}[ht]
    \centering
    \caption{The performance comparison with state-of-the-art methods on cityscapes.}
    \vspace{-5pt}
    % \begin{tabular}{m{2.0cm}<{\centering}|m{2.4cm}<{\centering}|m{3.6cm}<{\centering}|m{2.8cm}<{\centering}|m{2.8cm}<{\centering}|m{1.5cm}<{\centering}|m{1.5cm}<{\centering}|m{1.5cm}<{\centering}|m{1.5cm}<{\centering}}
    \begin{tabular}{c|m{3.0cm}<{\centering}|m{2.4cm}<{\centering}|m{2.4cm}<{\centering}|c|c|c|c}
    \toprule
    \multirow{2}{*}{Model} & \multirow{2}{*}{Method} &  \multirow{2}{*}{MACs} & \multirow{2}{*}{\#Params} & \multicolumn{4}{c}{@Limited Data~($\uparrow$)}\\
    \cline{5-8}
    &&&& 10\% & 25\% & 50\% & 100\% \\ 
    \hline 
    \multirow{8}{*}{Pix2Pix\cite{pix2pix}} 
    & Original-ResNet & 56.80G & 11.30M & & & & 44.32  \\
    \cline{2-8}
    & OMGD$_{\ 0.50\times}$ & 0.446G & 0.039M & & & & 37.65  \\
    & OMGD$_{\ 0.75\times}$ & 0.867G & 0.081M & & & & 42.15 \\
    & OMGD$_{\ 1.00\times}$ & 1.421G & 0.137M & & & & 45.21 \\
    \cline{2-8}
    & \multirow{3}{*}{UGC}  & 0.4G & M & & & & \\
    & & 0.8G & M & & & &  \\
    & & 1.4G & M & & & & \\
    \cline{2-8}
    & Original-UNet & 18.143G & 54.414M & & & & 42.71  \\
    \cline{2-8}
    & OMGD$_{\ 0.50\times}$ & 0.333G & 0.852M & & & & 41.54  \\
    & OMGD$_{\ 0.75\times}$ & 0.707G & 1.916M & & & & 45.52 \\
    & OMGD$_{\ 1.00\times}$ & 1.219G & 3.404M & & & & 48.91 \\
    \cline{2-8}
    & \multirow{3}{*}{UGC}  & 0.4G & M & & & & \\
    & & 0.8G & M & & & &  \\
    & & 1.4G & M & & & & \\
    \midrule
    \multirow{4}{*}{Pix2PixHD\cite{pix2pixhd}} 
    & Original & G & M & & & &  \\
    \cline{2-8}
    & \multirow{3}{*}{UGC}  & 0.4G & M & & & & \\
    & & 0.8G & M & & & &  \\
    & & 1.4G & M & & & & \\
    \midrule
    \multirow{4}{*}{GauGAN\cite{gaugan} } 
    & Original & 281.414G & 93.048M & 46.30 & 55.54 & 58.24 & 62.30 \\
    \cline{2-8}
    & \multirow{3}{*}{UGC}  & 0.4G & M & & & & \\
    & & 0.8G & M & & & & \\
    & & 1.4G & M & & & & \\
    \bottomrule
    \end{tabular}
    \vspace{-5pt}
    \label{table:result1} 
\end{table*}

==> tables/pseudo_algo.tex <==
\begin{algorithm}[t]
\footnotesize
    \caption{Unified GAN Compression Scheme.}
    \label{alg:1}
    \begin{algorithmic}[1]
    \State \textbf{Input:} 
    labeled dataset $\mathcal{A}$, unlabeled dataset $\mathcal{U}$, search space $ \mathcal{S}=\{G_i\} $, discriminator $D$, update interval $n$.
    \State \textbf{Output:} trained student generator $G^*$
    \State \textbf{\textit{Stage 1: Semi-Sup Network Architecture Search}}
    \State Initialize search space $\mathcal{S}$
    \For {$steps=1,...,T$}
        \State Sample $G_l$, $G_w$, $G_s$ from $\mathcal{S}$
        \State Sample a mini-batch data: $(x^{\mathcal{A}}, y^{\mathcal{A}})\in \mathcal{A}$, $x^{\mathcal{U}}\in \mathcal{U}$
        \State Calculate $\mathcal{L}^{\mathcal{A}}_{sup}(G_{l}, D)$ by Eq.\ref{eq:4}.
        \State Calculate $\mathcal{L}^{\mathcal{U}}_{dist}(G_{w}, G_{s})$ by Eq.\ref{eq:6}
        \State Update parameters of $G_l, G_s, G_w, D$.
    \EndFor
      
    \State \textbf{\textit{Stage 2: Adaptive Online Semi-Sup Distillation}}
    \State \textit{Evolutionary Architecture Search}: Search $G^*$, $G_{T}^{W}$, $G_{T}^{D}$ from $\mathcal{S}$  
    \State Initialize $G^*$, $G_{T}^{W}$, $G_{T}^{D}$, $D$ from \textit{Stage 1}.
    % \For {$epochs=1,...,T$}
    \For {$steps=1,...,T$}
        \State Sample a mini-batch data: $(x^{\mathcal{A}}, y^{\mathcal{A}})\in \mathcal{A}$, $x^{\mathcal{U}}\in \mathcal{U}$
        % \State $p_{t}^w=G_{T}^{W}(x)$; $p_{t}^d=G_{T}^{D}(x)$; $p_s=G_S(x)$
        \If{$steps$  $ \% $  $ n = 0$}
            \State Calculate $\mathcal{L}^{\mathcal{A}}_{sup}(G_{T}^{W}, D)$ by Eq.\ref{eq:4}.
            \State Calculate $\mathcal{L}^{\mathcal{A}}_{sup}(G_{T}^{D}, D)$ by Eq.\ref{eq:4}.
            \State Update parameters of $G_{T}^{W}$, $G_{T}^{D}$, $D$.
        \EndIf
        \State Calculate $\mathcal{L}_{dist}^{\mathcal{A}}(G^*)$ by Eq.\ref{eq:8}
        \State Calculate $\mathcal{L}_{dist}^{\mathcal{U}}(G^*)$ by Eq.\ref{eq:10}
        \State Update parameters of $G^*$
    \EndFor
    \end{algorithmic}
\label{alg:UGC} 
\end{algorithm}


==> tables/speed_wT4.tex <==
\begin{table}[ht]
\centering
\footnotesize
\caption{Latency Speedup.}
\vspace{-5pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{ccccm{1cm}<{\centering}m{1cm}<{\centering}m{1cm}<{\centering}}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{Method} & \multirow{2}{*}{MACs(G)} & \multicolumn{3}{c}{Latency(ms)}\\
\cline{4-6} 
 & & & Mi 10-CPU & Mi 10-GPU & Tesla T4 \\ 
\midrule
\multirow{4}{*}{Pix2Pix} 
& Original & 56.8 & 601 & 217.8 & 7.8 \\ 
\cline{2-6} 
 & GAN Com.\cite{GAN_compression} & 5.42(10.5$\times$) & 177.6(3.4$\times$) & 52.3(4.2$\times$) & 3.8(2.0$\times$) \\ 
 \cline{2-6} 
 & \multirow{2}{*}{UGC} & 1.50(38.0$\times$) & 92.3(6.5$\times$) & 34.1(6.4$\times$) & 3.2(2.4$\times$) \\ 
 \cline{3-6} 
 & & \textbf{0.89(63.6$\times$)}  & \textbf{60.7(9.9$\times$)} & \textbf{23.8(9.1$\times$)} & \textbf{3.5(2.2$\times$)} \\ 
 
\midrule

\multirow{4}{*}{GauGAN}  
 & Original & 281.4  & 2366.7 & 1252.5 & 26.9 \\ 
 \cline{2-6} 
 & GAN Com.\cite{GAN_compression} & 31.2(9.0$\times$) & 549.1(4.3$\times$) & 227.7(5.5$\times$) & 18.4(1.5$\times$) \\ 
 \cline{2-6} 
 & \multirow{2}{*}{UGC}  & 13.35(21.1$\times$)  & 332.5(7.1$\times$) & 155.8(8.0$\times$) & 11.3(2.4$\times$) \\ 
 \cline{3-6} 
 & & \textbf{9.51(29.6$\times$)}  & \textbf{275.6(8.6$\times$)} & \textbf{137.8(9.1$\times$)} & \textbf{10.5(2.6$\times$)} \\
\bottomrule
\end{tabular}
\renewcommand{\arraystretch}{1.}
\label{table:speed}
\end{table}
